Environment-Aware Dynamic Graph Learning for Out-of-Distribution Generalization

Dynamic graph neural networks (DGNNs) are increasingly pervasive in exploiting spatio-temporal patterns on dynamic graphs. However, existing works fail to generalize under distribution shifts, which are common in real-world scenarios. As the generation of dynamic graphs is heavily influenced by latent environments, investigating their impacts on the out-of-distribution (OOD) generalization is critical. However, it remains unexplored with the following two major challenges: (1) How to properly model and infer the complex environments on dynamic graphs with distribution shifts? (2) How to discover invariant patterns given inferred spatio-temporal environments? To solve these challenges, we propose a novel Environment-Aware dynamic Graph LEarning (EAGLE) framework for OOD generalization by modeling complex coupled environments and exploiting spatio-temporal invariant patterns. Specifically, we first design the environment-aware EA-DGNN to model environments by multi-channel environments disentangling. Then, we propose an environment instantiation mechanism for environment diversification with inferred distributions. Finally, we discriminate spatio-temporal invariant patterns for out-of-distribution prediction by the invariant pattern recognition mechanism and perform fine-grained causal interventions node-wisely with a mixture of instantiated environment samples. Experiments on real-world and synthetic dynamic graph datasets demonstrate the superiority of our method against state-of-the-art baselines under distribution shifts. To the best of our knowledge, we are the first to study OOD generalization on dynamic graphs from the environment learning perspective.

==> table/syn.tex <==
\begin{table}[htbp]
\label{tab:additional}
\caption{AUC  score (\% ± standard deviation) of future link prediction task on synthetic datasets. \textit{w/o OOD} and \textit{w/ OOD} denote testing without and with distribution shifts. $\mathbb{I}_{\mathrm{ACC}}$ is reported in the accuracy score). The best results are shown in $\mathbf{bold}$ and the runner-ups are \underline{$\rm{underlined}$}.}
\resizebox{\linewidth}{!}{
  \centering
  
    \begin{tabular}{c|c|c|cc|cc|cc}
    \toprule
    \multicolumn{2}{c|}{Shift Degree} & /     & \multicolumn{2}{c|}{$\bar{q}=$~0.4} & \multicolumn{2}{c|}{$\bar{q}=$~0.6} & \multicolumn{2}{c}{$\bar{q}=$~0.8} \\
    \midrule
    $\sigma_{\mathbf{e}}$     & Model & \textit{w/o OOD} & \textit{w/ OOD} & $\mathbb{I}_{\mathrm{ACC}}$  & \textit{w/ OOD} & $\mathbb{I}_{\mathrm{ACC}}$  & \textit{w/ OOD} & $\mathbb{I}_{\mathrm{ACC}}$  \\
    \midrule
    \multirow{2}[2]{*}{0.2} & DIDA  & 63.29±0.35 & 54.62±0.92 & /     & 53.33±1.01 & /     & 52.87±1.28 & / \\
          & \cellcolor[rgb]{ .91,  .91,  .91}\modelname & \cellcolor[rgb]{ .91,  .91,  .91}67.10±0.23 & \cellcolor[rgb]{ .91,  .91,  .91}59.91±1.18 & \cellcolor[rgb]{ .91,  .91,  .91}69.28±1.59 & \cellcolor[rgb]{ .91,  .91,  .91}54.71±1.29 & \cellcolor[rgb]{ .91,  .91,  .91}63.36±1.74 & \cellcolor[rgb]{ .91,  .91,  .91}54.26±1.31 & \cellcolor[rgb]{ .91,  .91,  .91}59.79±1.37 \\
    \midrule
    \multirow{2}[2]{*}{0.4} & DIDA  & 64.31±0.34 & 56.36±0.98 & /     & 56.04±1.13 & /     & 55.89±1.24 & / \\
          & \cellcolor[rgb]{ .91,  .91,  .91}\modelname & \cellcolor[rgb]{ .91,  .91,  .91}70.32±0.27 & \cellcolor[rgb]{ .91,  .91,  .91}63.97±0.82 & \cellcolor[rgb]{ .91,  .91,  .91}72.04±1.34 & \cellcolor[rgb]{ .91,  .91,  .91}61.08±1.02 & \cellcolor[rgb]{ .91,  .91,  .91}69.95±1.30 & \cellcolor[rgb]{ .91,  .91,  .91}58.40±1.12 & \cellcolor[rgb]{ .91,  .91,  .91}63.88±1.36 \\
    \midrule
    \multirow{2}[2]{*}{0.6} & DIDA  & 65.27±0.41 & 59.37±0.87 & /     & 58.79±0.97 & /     & 57.35±1.19 & / \\
          & \cellcolor[rgb]{ .91,  .91,  .91}\modelname & \cellcolor[rgb]{ .91,  .91,  .91}71.77±0.38 & \cellcolor[rgb]{ .91,  .91,  .91}66.01±0.74 & \cellcolor[rgb]{ .91,  .91,  .91}80.31±1.52 & \cellcolor[rgb]{ .91,  .91,  .91}63.26±0.64 & \cellcolor[rgb]{ .91,  .91,  .91}73.62±1.41 & \cellcolor[rgb]{ .91,  .91,  .91}63.11±0.78 & \cellcolor[rgb]{ .91,  .91,  .91}69.30±1.50 \\
    \midrule
    \multirow{2}[2]{*}{0.8} & DIDA  & 66.56±0.39 & 60.07±0.89 & /     & 59.82±1.05 & /     & 59.20±1.03 & / \\
          & \cellcolor[rgb]{ .91,  .91,  .91}\modelname & \cellcolor[rgb]{ .91,  .91,  .91}\underline{74.33±0.29} & \cellcolor[rgb]{ .91,  .91,  .91}\underline{68.41±0.72} & \cellcolor[rgb]{ .91,  .91,  .91}\underline{83.95±1.66} & \cellcolor[rgb]{ .91,  .91,  .91}\underline{66.15±0.69} & \cellcolor[rgb]{ .91,  .91,  .91}\underline{77.08±1.73} & \cellcolor[rgb]{ .91,  .91,  .91}\underline{65.82±0.81} & \cellcolor[rgb]{ .91,  .91,  .91}\underline{72.59±1.46} \\
    \midrule
    \multirow{2}[2]{*}{1.0} & DIDA  & 66.93±0.18 & 62.55±0.85 & /     & 61.05±0.93 & /     & 60.33±1.17 & / \\
          & \cellcolor[rgb]{ .91,  .91,  .91}\modelname & \cellcolor[rgb]{ .91,  .91,  .91}\textbf{75.58±0.40} & \cellcolor[rgb]{ .91,  .91,  .91}\textbf{70.12±0.91} & \cellcolor[rgb]{ .91,  .91,  .91}\textbf{85.83±1.54} & \cellcolor[rgb]{ .91,  .91,  .91}\textbf{69.83±0.93} & \cellcolor[rgb]{ .91,  .91,  .91}\textbf{79.56±1.65} & \cellcolor[rgb]{ .91,  .91,  .91}\textbf{68.09±0.97} & \cellcolor[rgb]{ .91,  .91,  .91}\textbf{74.16±1.21} \\
    \bottomrule
    \end{tabular}
}
\end{table}

